Resource-Constrained Robotic Planning in the face of Mixed Uncertainty

Robots operate under significant uncertainty, from quantifiable noise to unquantifiable unknowns, and must account for strict operational constraints, such as limited resources. In this paper, we consider the problem of synthesizing robust strategies to guide a robot's actions in fulfilling a given task, while ensuring the system never exhausts its resources. To solve this problem, we first model the robotic system as a Consumption Markov Decision Process with Set-valued Transitions(CMDPST), a unified framework modelling nondeterministic actions, quantifiable and unquantifiable uncertainty, and resource consumption. Then, we combine the CMDPST with the task specification, expressed as a Linear Temporal Logic over finite traces (LTLf ) formula. Lastly, we address the resource constrained optimal robust strategy synthesis problem, which aims to synthesize a strategy that maximizes the probability of satisfying the LTLf objective without resource exhaustion. Our solution involves two techniques: a direct unrolling-based method and a more efficient, optimized approach that leverages state-space pruning for better performance. Experiments on a warehouse transportation network show the effectiveness of the proposed solutions.

==> LP_algorithm.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\capvar}{\text{cap}}
% \newcommand{\cost}{\text{cost}}
\newcommand{\init}{\text{init}}


\czm{I have added a section on solving MDP reachability probability problems under energy constraints using both linear programming and multi-objective linear programming.}
\section{Linear Programming for Maximum Reachability under Energy Constraints with Recharging}
\label{sec:lp-formulation}

We consider the problem of computing the maximum probability of reaching a target set $ F \subseteq S $ in a finite-state Markov decision process (MDP) with energy constraints and recharging capabilities. The system is modeled as an \emph{consumption MDP} $ \mathcal{M} = (S, A, P, R, \cost, \capvar, F, \alpha) $, where:
\begin{itemize}
    \item $ S $ is a finite state set, $ F \subseteq S $ is absorbing;
    \item $ A(s) $ is the finite action set at $ s \in S $;
    \item $ P(s' \mid s,a) $ is the transition probability;
    \item $ R \subseteq S $ is the set of \emph{recharging stations}: upon entering $ s' \in R $, energy is reset to $ \capvar \in \Z_{>0} $;
    \item $ \cost: S \times A \to \Z_{>0} $ assigns strictly positive energy costs;
    \item $ \alpha: S \setminus F \to [0,1] $ is the initial state distribution, with full initial energy.
\end{itemize}

Due to recharging, infinite paths avoiding $ F $ may exist, preventing direct use of undiscounted flows. To ensure boundedness, we introduce a discount factor $ \gamma \in (0,1) $ and formulate the problem as the following linear program over occupation measures~\cite{Pitman_1977} $ x(s,e,a) $, representing the expected discounted number of times action $ a $ is taken in state $ s $ with energy $ e $.

\begin{subequations}
\label{lp:main}
\begin{align}
    \max_{x \geq 0} \quad & \sum_{s \in S \setminus F} \sum_{e \in E} \sum_{a \in A(s)} \sum_{s' \in F} P(s' \mid s,a) \cdot x(s,e,a) 
    \label{lp:obj} \\
    \text{s.t.} \quad & \sum_{a' \in A(s')} x(s',e',a') 
    = 
    \delta_{e',\capvar} \alpha(s') 
    + \notag \\
    & \gamma \sum_{s \in S \setminus F} \sum_{a \in A(s)} P(s' \mid s,a) \cdot I(s', e', s, a), 
    \notag \\
    & \hspace{5em} \forall (s', e') \in (S \setminus F) \times E,
    \label{lp:flow}
\end{align}
\end{subequations}
where $ E = \{0,1,\dots,\capvar\} $, and the inflow term $ I(s', e', s, a) $ is defined as:
\begin{equation}
    I(s', e', s, a) =
    \begin{cases}
        x(s, e' + \cost(s,a), a) 
        & \text{if } s' \notin R \text{ and } e' + \cost(s,a) \leq \capvar, \\
        \sum_{e \geq \cost(s,a)} x(s,e,a) 
        & \text{if } s' \in R \text{ and } e' = \capvar, \\
        0 & \text{otherwise}.
    \end{cases}
    \label{eq:inflow}
\end{equation}

Constraint~\eqref{lp:flow} enforces \emph{discounted flow conservation} in the augmented state space $ (S \setminus F) \times E $: the total outflow from $ (s',e') $ equals the initial injection (only at full energy) plus the discounted inflow from predecessors, adjusted for energy consumption and recharging. The inflow in~\eqref{eq:inflow} correctly models energy cost and instantaneous recharge upon entering $ R $. The objective~\eqref{lp:obj} sums the probability transferred into target set $ F $, which equals the total probability of entering F from $S \setminus F$ for first time under the induced policy.

We now establish the correctness of this formulation.

\begin{theorem}[Asymptotic Optimality]
Let $ \mathcal{P}^* $ denote the maximum probability of reaching $ F $. Let $ \mathrm{OPT}(\gamma) $ be the optimal value of LP~\eqref{lp:main}. Then:
\[
    \lim_{\gamma \to 1^-} \mathrm{OPT}(\gamma) = \mathcal{P}^*.
\]
\end{theorem}

\begin{proof}
We first show $ \mathrm{OPT}(\gamma) \leq \mathcal{P}^* $. For any policy $ \pi $, its induced occupation measure $ x^\pi $ satisfies~\eqref{lp:flow}, and the objective evaluates to $ J_\gamma(\pi) = \E_\pi[\sum_{t=0}^\infty \gamma^t \mathbf{1}_{(s_t \notin F, s_{t+1} \in F)}] \leq \Pb_\pi(\lfinally F) \leq \mathcal{P}^* $. Thus $ \mathrm{OPT}(\gamma) \leq \mathcal{P}^* $.

Next, let $ \pi^* $ be an optimal policy with $ \Pb_{\pi^*}(\lfinally F) = \mathcal{P}^* $. Let $ T = \min\{ t \geq 0 : s_t \in F \} $ ($ T = \infty $ if $ F $ is never reached). Then $ J_\gamma(\pi^*) = \E_{\pi^*}[\gamma^T \cdot \mathbf{1}_{T < \infty}] $. As $ \gamma \to 1^- $, $ \gamma^T \uparrow 1 $ on $ \{T < \infty\} $, $ \lim_{\gamma \to 1^-} J_\gamma(\pi^*) = \mathcal{P}^* $. Since $ J_\gamma(\pi^*) \leq \mathrm{OPT}(\gamma) \leq \mathcal{P}^* $, the result follows.
\end{proof}

This formulation enables efficient approximation of $ \mathcal{P}^* $ via standard LP solvers. The optimal policy can be recovered from the solution $ x^* $ via:
\[
    \pi^*(a \mid s,e) = \frac{x^*(s,e,a)}{\sum_{a' \in A(s)} x^*(s,e,a')}
\]
where $\sum_{a' \in A(s)} x^*(s,e,a') \neq 0$, otherwise $\pi^*(a \mid s,e) = 0$.
In practice, choosing $ \gamma $ close to 1 (e.g., $ 0.999 $) yields high-precision estimates of the true reachability probability.


\section{Extension to Multi-Objective Reachability}
\label{sec:multi-objective}

We now extend the single-objective formulation to the \emph{multi-objective probabilistic reachability} problem, where the goal is to simultaneously satisfy multiple probabilistic thresholds for reaching different target sets. This setting arises in safety-critical systems with multiple correctness or liveness requirements.

Let $ F_1, F_2, \dots, F_k \subseteq S $ be $ k $ distinct target sets, with $ F = \bigcup_{i=1}^k F_i $ and each state $ v \in F $ being \emph{absorbing}. Let $ \alpha \in \mathcal{D}(S \setminus F) $ be an initial distribution over non-target states (with $ S \setminus F \neq \emptyset $), and let $ r = (r_1, \dots, r_k) \in (0,1]^k $ be a vector of required success probabilities. The multi-objective problem asks whether there exists a strategy $ \sigma $ such that:
\[
    \bigwedge_{i=1}^k \left( \Pr\nolimits_\alpha^\sigma(\Diamond F_i) \geq r_i \right),
\]
where $ \Pr_\alpha^\sigma(\Diamond F_i) $ denotes the probability of eventually reaching $ F_i $ under strategy $ \sigma $ from initial distribution $ \alpha $.

Building upon the single-objective LP formulation in Section~\ref{sec:lp-formulation}, we define a \emph{multi-objective discounted linear program} that captures all objectives simultaneously. As before, we use a discount factor $ \gamma \in (0,1) $ to ensure boundedness under recharging dynamics.

\begin{subequations}
\label{lp:multi}
\begin{align}
    \max \quad & x(s,e,a) \geq 0, \quad \forall s \in S \setminus F,\, e \in E,\, a \in A(s) \\
    \text{s.t.} \quad & \sum_{a' \in A(s')} x(s',e',a') 
    = 
    \delta_{e',\capvar} \alpha(s') 
    + \notag\\
    & \gamma \sum_{s \in S \setminus F} \sum_{a \in A(s)} P(s' \mid s,a) \cdot I(s', e', s, a), 
    \notag \forall (s', e') \in (S \setminus F) \times E,\\
    \label{lp:multi-flow} \\
    & \sum_{s \in S \setminus F_i} \sum_{e \in E} \sum_{a \in A(s)} \sum_{s' \in F_i} P(s' \mid s,a) \cdot x(s,e,a) \geq r_i,
    \forall i = 1,\dots,k,
    \label{lp:multi-threshold}
\end{align}
\end{subequations}
where the inflow function $ I(\cdot) $ is defined as in~\eqref{eq:inflow}. The constraints~\eqref{lp:multi-flow} enforce discounted flow conservation across the energy-augmented state space, while~\eqref{lp:multi-threshold} impose lower bounds on the flow into each target set $ F_i $.

We now state a fundamental result, adapted from~\cite{EtessamiKVY14} and generalized to energy-constrained systems with recharging, which establishes the equivalence between strategy existence and LP feasibility.

\begin{theorem}[Multi-Objective Strategy Characterization]
\label{thm:multi-objective}
The following are equivalent:
\begin{enumerate}
    \item[(1)] There exists a (possibly randomized) memoryless strategy $ \sigma $ such that
    \[
        \bigwedge_{i=1}^k \left( \Pr\nolimits_\alpha^\sigma(\Diamond F_i) \geq r_i \right).
    \]
    \item[(2)] There exists a feasible solution $ x $ to the multi-objective LP~\eqref{lp:multi} such that
    \[
        \bigwedge_{i=1}^k \left( \sum_{s \in S \setminus F_i} \sum_{e,a,s'} P(s' \mid s,a) \cdot x(s,e,a) \geq r_i \right).
    \]
    when $\gamma \to 1^-$
    \item[(3)] There exists an arbitrary (history-dependent, infinite-memory) strategy $ \sigma $ such that
    \[
        \bigwedge_{i=1}^k \left( \Pr\nolimits_\alpha^\sigma(\Diamond F_i) \geq r_i \right).
    \]
\end{enumerate}
\end{theorem}

\begin{proof}[Proof Sketch]
The implication (1) $ \Rightarrow $ (3) is trivial. (3) $ \Rightarrow $ (2) follows by constructing the discounted occupation measure $ x^\sigma(s,e,a) = \E_\sigma[\sum_{t=0}^\infty \gamma^t \mathbf{1}_{(s_t=s,e_t=e,a_t=a)}] $ from any strategy $ \sigma $ satisfying (3), which satisfies the flow constraints~\eqref{lp:multi-flow} and the threshold constraints~\eqref{lp:multi-threshold} in the limit as $ \gamma \to 1^- $. For $ \gamma $ sufficiently close to 1, the discounted flow into $ F_i $ approximates $ \Pr_\alpha^\sigma(\Diamond F_i) $, ensuring feasibility.

The key direction (2) $ \Rightarrow $ (1) relies on the fact that any feasible $ x $ induces a \emph{randomized memoryless} strategy via:
\[
    \sigma(a \mid s,e) = \frac{x(s,e,a)}{\sum_{a' \in A(s)} x(s,e,a')}, \quad \text{if } \sum_{a'} x(s,e,a') > 0.
\]
For (3) $ \Rightarrow $ (1), it can follows the
proof in ~\cite{EtessamiKVY14}).

Thus, the three conditions are equivalent.
\end{proof}

% \begin{remark}
% The use of discounting $ \gamma < 1 $ is again essential to handle infinite paths enabled by recharging. However, as shown in the proof, the existence of a feasible solution for $ \gamma $ arbitrarily close to 1 implies the existence of a memoryless strategy achieving the exact (undiscounted) probabilities. This allows us to use the discounted LP as a sound and complete witness for multi-objective reachability.
% \end{remark}

This result enables the use of linear programming to solve multi-objective model checking problems under energy constraints. One can iteratively solve~\eqref{lp:multi} for increasing $ \gamma \to 1^- $ to verify whether a given requirement vector $ r $ is achievable. If feasible, a corresponding memoryless strategy is directly extracted from the solution.

==> sections/computer_winning_region.tex <==
\section{Optimized Robust Strategy Synthesis}
\label{sec:strategySynthesis}


In the previous section, we introduced the unrolled approach to convert a CMDPST $\mdpst^{\times}$ to an MDPST $\mdpst^{\unrolled}$ which records the current resource level in each state.
This na\"ive approach not only hinders the scalability of our synthesis approach but also yields an optimal robust strategy of large size.
To this end, we propose to first prune the CMDPST $\mdpst^{\times}$ before converting to the MDPST.
That is, we will remove all states from which the agent does not have a strategy to accomplish the task. 

%In this section, we introduce an solution to check whether there exists a feasible strategy given a CMDPST $\mdpst$ and a set $T$ of target states.
We observe that the approach we present in this section can also be used in the design phase of the system to check whether there exists a feasible strategy given a CMDPST $\mdpst$ and a set $T$ of target states.
That is, when deploying a system to complete a task, it is often necessary to check first whether the current system has a feasible strategy instead of computing an optimal robust strategy directly.
Any deployment error found in this phase can be fixed immediately.
For instance, once we find out that there are no feasible strategies, we can look for the root causes, such as that there are not enough charging stations or the geometric distribution of the charging stations is not reasonable in our warehouse example, so we can add more or adjust the locations of the charging stations in order to fulfill the given (set of) task(s).

Another advantage of our proposed optimization is that it only involves simple graph exploration and value iteration.
Thus, it is easy to implement.
The central idea in our optimization is to compute the winning region where the agent has a strategy to reach the target states $T$ against any nature.
So for feasibility check, we can then test whether from the initial state, the agent has a strategy to reach the winning region.
And for pruning, we only need to remove all states that can not reach the target area.
% \begin{enumerate}
%     \item construct a DFA $\dfa_{\varphi}$ from $\varphi$ such that $\lang(\dfa_{\varphi}) = [\varphi]$,
%     \item build the product CMDPST $\mdpst^{\times}$ of $\mdpst$ and $\dfa_{\varphi}$,
%     \item analyze the product CMDPST $\mdpst^{\times}$, and
%     \item compute the robust strategy.
% \end{enumerate}

% \ly{We need to figure out why we need to compute the winning region. From the current experiments, we do not have a reason for that.}
%it first computes the winning region for the problem and then synthesizes and extracts the optimal strategy that maximizes the satisfaction of the given $\ltlf$ formula $\varphi$.



% \subsection{Compute the winning region}
Our input here is the product CMDPST $\mdpst^{\times}$ constructed in Section~\ref{sec:unroll}. 
Nonetheless, to make the presentation more general, we assume that we are given a CMDPST $\mdpst = (S, \bar{s}, A, \mathcal{F}, \mathcal{T}, L, C, R, \rcap)$ and a set of target states $T \subseteq S$.
% Due to limited resource capacity and nondeterministic transitions, we cannot rely on classical MDP planning techniques that assume expected value updates or fixed probabilistic dynamics, since we also have to consider the uncertainty in the choice of the successor state and the need to not exceed the resource consumption limits.
% This means that we must ensure that the synthesized strategy remains valid under the worst-case resolutions of set-valued transitions.
% To address this challenge, we introduce the concept of the \emph{winning region}, which characterizes the set of states that can contribute to the satisfaction of the task under some feasible strategy.

% \begin{definition}[Winning region]
% Given a CMDPST $\mdpst$ and a set of target states $T \subseteq S$, the \emph{winning region} $W \subseteq S$ is the set of states that satisfy one of the following conditions:
% \begin{itemize}
% \item 
%     There exists a strategy $\strategy$ such that every $t \in T \cap W$ is reachable from $\bar{s}$ along some finite execution path under $\strategy$.
% \item 
%     For each reload state $r \in R \cap W$, there must exist a strategy $\strategy$ such that, under worst-case transition choices, some target state $t \in T$ is reachable from $r$, and $r$ itself is reachable from the initial state $\bar{s}$ via a finite path under $\strategy$.
% \end{itemize}
% \end{definition}

%\py{"worst-case transition choices" is not completely clear to me. When introduce MDPST in Section 3, add the definition of "Robust Strategy". Then here we can say "there exists a robust strategy..."}

To deal with the resource constraints, we first compute for each state its minimal resource consumption to reach a target state in $T$, then we compute the set of all valid reload states, i.e., the reload states that have a minimal resource consumption below $\rcap$ to reach the target states or another valid reload state, and finally we compute the winning region where each state can reach a target state or a valid reload state with probability one, independently of nature's choices.

\subsubsection{Minimal Resource consumption}

\begin{algorithm}
\caption{\proc{MinResCons}}
\label{alg:minResCons}
\begin{algorithmic}[1]
    \Require CMDPST $\mdpst$, target states $T$
    \State initialize $\Vec{x} \in \naturals^{S}$ to be $\infty$ in every component
    \ForAll{$t \in T$}
        % \State 
        $\Vec{x}(t) \gets 0$
    \EndFor
    \Repeat
        \State $\Vec{x}^{\text{prev}} \gets \Vec{x}$
        \ForAll{$s \in S \setminus T$}
            % \State 
            $\Vec{x}(s) \gets \mathit{min\_max}(s)$
        \EndFor
    \Until{$\Vec{x}^{\text{prev}} = \Vec{x}$}
    \State \Return $\Vec{x}$
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:minResCons} calculates the minimal resource consumption for each state to reach a target state against any adversarial nature.
Note that \proc{MinResCons} ignores the role of reload states, which is taken into consideration by the algorithms \proc{ValidReloadStates} and \proc{WinningRegion} presented below and that call \proc{MinResCons} on different sets $T$. 

\proc{MinResCons} updates the resource requirement upper bounds through value iteration. 
All states' initial resource consumption $\Vec{x}(s)$ is initialized to $\infty$ and the resource consumption of each target state $t \in T$ is reset to $0$, i.e., $\Vec{x}(t) \gets 0$.
Then, until convergence is reached ($\Vec{x}^{\text{prev}} = \Vec{x}$), for each non-target state $s \notin T$, its value is updated using $\mathit{min\_max}(s)$:
\[
    \mathit{min\_max}(s) = \min_{a \in A(s)} \Big( C(s, a) + \max_{\Theta \in \mathcal{F}(s, a)} \max_{s' \in \Theta} \Vec{x}(s') \Big)
\]
where $C(s, a)$ is the immediate resource consumption for executing action $a$ in state $s$, $\mathcal{F}(s, a)$ is the set-valued transition function for action $a$ in state $s$, and $\max_{\Theta} \max_{s' \in \Theta} \Vec{x}(s')$ represents nature choosing the worst-case transition set $\Theta$ and selecting the successor state $s'$ with the highest resource consumption.
% \ly{I would say that the probable player chooses the $\Theta$ and $s'$ is chosen by nature, of course we see probaly player as adversarial player also. }
Lastly, the final $\Vec{x}$ is returned, where $\Vec{x}(s)$ gives the minimal resource required to reach $T$ when starting from state $s$. 
Theorem~\ref{thm:correctnessMinResCons} provides the correctness of Algorithm~\ref{alg:minResCons}.

\begin{theorem}
\label{thm:correctnessMinResCons}
    Given a CMDPST $\mdpst$ and a set of target states $T$, let $\Vec{x} = \proc{MinResCons}(\mdpst, T)$.
    Then, for each $s \in S$, either $s \in T$ and $\Vec{x}(s) = 0$, or there exists a strategy $\strategy$ such that for each finite path $\fpath = s_{0} a_{0} \dots s_{n} \in \fpaths$ with $s_{0} = s$, $s_{n} \in T$, and $s_{i} \notin T$ for each $0 \leq i < n$, if $\prob^{\strategy}_{s}(\{\fpath\}) > 0$, then $\cost(\fpath) \leq \Vec{x}(s)$.
\end{theorem}
\begin{proof}
For target states \( t \in T \), \( \Vec{x}(t) = 0 \) is correct since we have reached the final region and no resources are needed thereafter.
For non-target states $s \notin T$, the algorithm updates $\Vec{x}(s)$ using the formula:
\[
\Vec{x}(s) = \min_{a \in A(s)} \Big( C(s, a) + \max_{\Theta \in \mathcal{F}(s, a)} \max_{s' \in \Theta} \Vec{x}(s') \Big)
\]
The outer $\min_{a}$ ensures the strategy selects the optimal action, while the inner double $\max$ simulates the worst-case transitions chosen by nature.
%\at{The following should be the inductive step, as this proof is like a proof by induction on the number of steps before reaching the fix point.}
%If $x(s')$ correctly represents the minimal resource requirements for successor states $s'$, then $x(s)$ accounts for all possible adversarial choices, thereby ensuring safety.
%Since each iteration of $x(s)$ is monotonically decreasing and bounded below (by non-negativity), the algorithm converges to the least fixed point.


Consider any finite path $\fpath = s_{0} a_{0} \dots s_{n}$ with $s_{0}=s$, $s_{n}\in T$, and $s_{i}\notin T$ for $0 \leq i < n$. The cost of such a path can be written as
\[
\cost(\fpath) = \sum_{i=0}^{n-1} C(s_{i},a_{i}).
\]
Suppose that for all successor states $s'$ the values $\Vec{x}(s')$ already bound from above the minimal resource consumption of any path from $s'$ to $T$. Then, for any action $a$ and any worst-case choice of successor $s'$, the accumulated cost along $\fpath$ satisfies
\[
\cost(\fpath) \leq C(s,a) + \Vec{x}(s').
\]
Taking the worst case over all possible successors and then the best action yields exactly the update rule above, showing that $\Vec{x}(s)$ bounds the minimal resource required from $s$.  

Since the updates monotonically decrease $\Vec{x}(s)$ and are bounded below by $0$, the iteration converges to the least fixed point. At this point, $\Vec{x}(s)$ coincides with the minimal resource consumption needed to reach $T$ from $s$ without exhausting resources under adversarial choices.  
\at{Do we have some guarantee about the number of iterations the algorithm can take at most?}
\py{Yes, I believe the maximum number of iterations needed is the maximal steps $T_{max} < |S^{\times}|$ needed to reach the target set.}

%\ly{Andrea already suggested to formalize the proof more precisely with inductive steps. Please do so. Also, in the proof, you did not even mention $\cost$ function. We need to explicitly do it.}
\end{proof}





\subsubsection{Computing the valid reload states}


\begin{algorithm}
\caption{\proc{ValidReloadStates}}
\label{alg:validReloadStates}
\begin{algorithmic}[1]
    \Require CMDPST $\mdpst$
    \State Initialize $\text{Rel}_{\text{valid}} \gets \emptyset$

    \Repeat
        \State $\text{Rel}_{\text{valid}}^{\text{prev}} \gets \text{Rel}_{\text{valid}}$
        \ForAll{$r \in R \setminus \text{Rel}_{\text{valid}}$}
            \State $\Vec{x} \gets \proc{MinResCons}(\mdpst, \{r\})$ 
            \If{$\Vec{x}(\bar{s}) \leq \rcap$ or there is $r' \in \text{Rel}_{\text{valid}}$ such that $\Vec{x}(r') \leq \rcap$}
                \State $\text{Rel}_{\text{valid}} \gets \text{Rel}_{\text{valid}} \cup \{r\}$
            \EndIf
        \EndFor
    \Until{$\text{Rel}_{\text{valid}}^{\text{prev}} = \text{Rel}_{\text{valid}}$}

    \State \Return $\text{Rel}_{\text{valid}}$
\end{algorithmic}
\end{algorithm}

The objective of Algorithm~\ref{alg:validReloadStates} is to identify a subset of reload states, $\text{Rel}_{\text{valid}}$, that are either directly reachable from the initial state $\bar{s}$ with some feasible strategy or can be visited from other such reload states.
To this end, we iteratively apply Algorithm~\ref{alg:minResCons} to check whether a reload state $r \in \text{Rel}$ is reachable with some strategy from either the initial state $\bar{s}$ or from any already validated reload state $r' \in \text{Rel}_{\text{valid}}$ without exceeding the resource capacity $\rcap$. 
At each iteration, validated reload states are added to $\text{Rel}_{\text{valid}}$. 
The process continues until a fixed point is reached, i.e., no more new valid reload states are discovered. 
% This iterative expansion ensures that all reload states that are transitively reachable via secure replenishment paths are correctly identified.






\subsubsection{Extracting the winning region}


\begin{algorithm}[b]
\caption{\proc{WinningRegion}}
\label{alg:winningRegion}
\begin{algorithmic}[1]
    \Require CMDPST $\mdpst$, target states $T$
    \State $\text{Rel}_{\text{valid\_new}} \gets \emptyset$; $T_{\text{safe}} \gets \emptyset$%; $\text{NewAdded} \gets \text{True}$
    \State $\text{Rel}_{\text{valid}} \gets \proc{ValidReloadStates}(\mdpst)$ ;
    \ForAll{$t \in T$}
        \State $\Vec{x} \gets \proc{MinResCons}(\mdpst, \{t\})$
        \If{$\Vec{x}(\bar{s}) \leq \rcap$}
            $T_{\text{safe}} \gets T_{\text{safe}} \cup \{t\}$
        \EndIf
    \EndFor
    \State $T \gets T_{\text{safe}}$
    \Repeat
        \State $\text{Rel}_{\text{valid\_new}}^{\text{prev}} \gets \text{Rel}_{\text{valid\_new}}$
    % \While{$\text{NewAdded}$}
        % \State $\text{NewAdded} \gets \text{False}$
        \ForAll{$r \in \text{Rel}_{\text{valid}} \setminus \text{Rel}_{\text{valid\_new}}$}
            \State $\Vec{x} \gets \proc{MinResCons}(\mdpst, T)$
            \If{$\Vec{x}(r) \leq \rcap$}
                \State $\text{Rel}_{\text{valid\_new}} \gets \text{Rel}_{\text{valid\_new}} \cup \{r\}$
                \State $T \gets T \cup \{r\}$
                % \State $\text{NewAdded} \gets \text{True}$
            \EndIf
        \EndFor
    % \EndWhile
    \Until $\text{Rel}_{\text{valid\_new}}^{\text{prev}} = \text{Rel}_{\text{valid\_new}}$
    
    \State $W \gets T_{\text{safe}} \cup \text{Rel}_{\text{valid\_new}}$
    \State \Return $(x, W, \text{Rel}_{\text{valid\_new}}, T_{\text{safe}})$
    %\State $W \gets T_{\text{safe}} \cup \text{Rel}_{\text{valid}}$
    %\State \Return $(x, W, \text{Rel}_{\text{valid}}, T_{\text{safe}})$
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:winningRegion} computes a refined winning region from which the agent has some strategy to reach the target set under the resource constraints.
Its purpose is twofold:
\begin{itemize}
    \item filter out unreachable target states that cannot be reached from the initial state $\bar{s}$ within the resource capacity;
    \item identify reload states that can contribute to reaching these filtered target states while maintaining feasibility against the adversarial nature.
\end{itemize}

% \ly{Do we stick to worst-case transitions, worst-case resource consumption, worst-case adversarial resolution within the resource limit, worst-case resolution of nondeterminism, or under the most adversarial environmental transitions?}

The algorithm proceeds in two major phases:

\paragraph{Initial target filtering}
For each candidate target state $t \in T$, it computes the minimum resource consumption required to reach $t$ from the initial state $\bar{s}$ against any nature using \proc{MinResCons}.
Only the states $t$ under resource constraints, i.e., with $\Vec{x}(\bar{s}) \leq \rcap$ are retained as safe target states $T_{\text{safe}}$.

\at{There is something I don't get here: why at line 6 the original target states $T$ are replaced by the ones that can be directly reached from the initial state within the resource constraint? What if there are no such states? $T_{\text{safe}}$ is empty, so is $T$, thus $\Vec{x} \gets \proc{MinResCons}(\mdpst, T)$ at line 10 is filled with $\infty$, the repeat loop terminates immediately and $W$ only contains the valid reload states.}
\yh{I think the set T in line 10 should be the original target states, not the one computed in line 6.}
\at{If it is the original, then the vector is always the same, so the loop is essentially useless. I think there are other, deeper changes to be applied to the algorithm to make it correct}
\yh{The original target states are the ones we actually want to reach. As long as a reload state can reach any one of these original targets, it should be kept. Therefore, replacing the current target set with the original one seems reasonable to me. If this makes the loop redundant, we can simply remove it.What do you think}
\at{But then you don't consider the role of reload states that should be part of the winning region. Moreover, the winning region is going to miss all intermediate non-reload states that are between the initial/reload states and the target states (which should be there, according to the intuitive description of winning region at the beginning of the section. As a concrete example: take the CMDPST that is just the chain $s_{0} \xrightarrow{a} s_{1} \xrightarrow{a} s_{2} \xrightarrow{a} s_{3} \xrightarrow{a} s_{4}$. Each transition costs 1, $\rcap = 3$, $R = \{s_{2}\}$, $T = \{s_{4}\}$. What is the winning region $W$ here? I would say $W = S$, but the algorithm gives what?}
\yh{I think that WR is merely a rephrasing of the target state, divided into direct and indirect reachability. Direct reachability means arriving without considering the effect of reload states, starting from the initial state. Indirect reachability means arriving via reload states. As long as the retained reload states can reach one of the original target states, we can treat those reload states as target states themselves. Therefore, I think WR is just another way of describing target states that account for the role of reload states, and should not include any other ordinary states.In the example you gave, the winning region should only contain S2}
\at{If this is the interpretation of winning region, then this is what needs to be written in the draft, not the current version}


\paragraph{Reload state filtering and iterative refinement}
Using the reload set $\text{Rel}_{\text{valid}}$ extracted by \proc{ValidReloadStates}, the algorithm iteratively checks each reload state $r$ to see whether $r$ can reach some target in the current $T$ (starting with $T_{\text{safe}}$) against any nature within the resource limit.
If so, the reload state is added to the refined reload set $\text{Rel}_{\text{valid\_new}}$ and appended to the target set $T$ for further propagation. This process continues until no new reload states are added.

Finally, the winning region $W$ is defined as the union of all surviving target states and the newly added reload states:
\[
    W = T_{\text{safe}} \cup \text{Rel}_{\text{valid\_new}}.
\]
represents the set of states from which the task can be safely fulfilled. 
Reaching a state in $T_{\text{safe}}$ means that the target is already accomplished within the resource bound, 
while reaching a state in $\text{Rel}_{\text{valid\_new}}$ guarantees that the agent can replenish its resources 
and subsequently reach a safe target. 
Thus, any run that enters $W$ ensures the feasibility of completing the task under the given constraints.
%\ly{We need more explanation for this winning region.}
\ly{Is this theorem also complete?}
\begin{theorem}[Correctness of Target and Reload Filtering]
    Let $W$ be the output winning region computed by Algorithm~\ref{alg:winningRegion}. 
    Then for every state $s \in W$, there exists a strategy $\strategy$ such that starting from $\bar{s}$, under the worst-case resolution of nondeterminism, the system can reach $s$ within the resource limit $\rcap$, and $s$ can further reach some goal state (possibly itself) also within $\rcap$.
\end{theorem}

\begin{proof}
The algorithm includes a state $t$ in $T_{\text{safe}}$ only if the worst-case resource cost from $\bar{s}$ to $t$ does not exceed $\rcap$. This ensures feasibility of reaching $t$ directly from the initial state.

For each reload state $r \in \text{Rel}_{\text{valid}}$, the algorithm checks whether the minimum required resource to reach the current target set $T$ from $r$ is within the capacity bound.
Only those states satisfying this property are added to $\text{Rel}_{\text{valid\_new}}$ and to the expanding target set $T$.

By induction over the iterations:

In the first round, all states in $T_{\text{safe}}$ are reachable from $\bar{s}$ within capacity.

In each subsequent round, a reload state $r$ is added only if it can reach some state already in $T$ within capacity, thus ensuring a valid resource-feasible path from $r$ to target states.

Since all $r \in \text{Rel}_{\text{valid}}$ are reachable from $\bar{s}$ by definition of \proc{ValidReloadStates}, and all $r \in \text{Rel}_{\text{valid\_new}}$ are guaranteed to be able to reach $T$, it follows that there exists a valid strategy from $\bar{s}$ to reach a goal via such $r$.

Therefore, for any $s \in W$, the system can safely reach $s$ from the initial state and eventually reach a goal state, without violating the resource constraint.
\end{proof}



If a reload state admits a resource-feasible path to an accepting state, and the initial state can safely reach that reload state, then the initial state is effectively connected to the target states via a valid plan. 
Thus, such reload states are incorporated into the winning region.



\iffalse
\subsection{Synthesize and Extract the Optimal Robust Strategy}

In order to compute the winning region, we ween to identify the set of target states that correspond to the satisfaction by the paths of $\mdpst$ of the given $\ltlf$ formula $\varphi$.
We identify such target states by the usual product automaton $\mdpst \times \dfa_{\varphi}$ adapted to the CMDPST model.

\begin{definition}[Product CMDPST]
\label{def:productCMDPST}
    Given a CMDPST $\mdpst = (S, \bar{s}, A, \mathcal{F}, \mathcal{T}, L, C, R, \rcap)$ and an $\ltlf$ formula $\varphi$, let $\dfa_{\varphi} = (\Sigma, Q, \bar{q}, \delta, \acc)$ be its corresponding DFA. 
    The \emph{product CMDPST} $\mdpst^{\times}$ is defined as
    \[
        \mdpst^{\times} = (S^{\times}, \bar{s}^{\times}, A^{\times}, \mathcal{F}^{\times}, \mathcal{T}^{\times}, L^{\times}, C^{\times}, R^{\times}, \rcap^{\times}, \acc^{\times})
    \]
    where:
    \begin{itemize}
    \item 
        $S^{\times} = S \times Q$ and $\bar{s}^{\times} = (\bar{s}, \bar{q})$;
    \item 
        $A^{\times} = A$;
    \item
        $\mathcal{F}^{\times}$ and $\mathcal{T}^{\times}$ are defined as follows:
        for each $(s, q) \in S^{\times}$ and $a\in A^{\times}$, let $q' = \delta(q, L(s))$. 
        Then $\mathcal{F}^{\times}((s, q), a) = \setcond{\Theta \times \{q'\}}{\Theta \in \mathcal{F}(s, a)}$ and, for each $\Theta \in \mathcal{F}(s, a)$, $\mathcal{T}^{\times}((s, q), a, \Theta \times \{q'\}) = \mathcal{T}(s, a, \Theta)$;
    \item 
        $L^{\times}((s, q)) = L(s)$ for each $(s, q) \in S^{\times}$;
    \item 
        $C^{\times}((s, q), a) = C(s, a)$;
    \item 
        $R^{\times} = \setcond{(s,q) \in S^{\times}}{s \in R}$;
    \item 
        $\rcap^{\times} = \rcap$; and
    \item 
        $\acc^{\times} = \setcond{(s, q) \in S^{\times}}{q \in \acc}$.
    \end{itemize}
\end{definition}

Based on the constructed product CMDPST $\mdpst^{\times}$ and the identified winning region $W$ for the target states $\acc^{\times}$, we now focus on synthesizing an optimal strategy that guarantees the satisfaction of the $\ltlf$ specification $\varphi$ under worst-case transition behaviors.
Since the specification is defined over finite traces, the strategy synthesis problem reduces to computing a policy that maximizes the probability of reaching the winning region $W$ from the initial state $\bar{s}^{\times}$.

\at{Changed section up to here. Problems below still need to be discussed}

\at{In the definition below, we don't use the fact that the model is a product CMDPST. So we could just use a MDPST. Unless we start enforcing requirements like the strategy being feasible/robust. Anyway the product is not needed, as we only use the winning region. Also, robust strategies are defined wrt.\@ some $\beta$ that is missing here\dots}


\fi

\at{Right now, the concept of winning region is too polluted and it seems we are trying to stretching it to do too many things. What follows is my proposal for computing the feasible area, instead of the winning region, as in the motivation at the beginning of the section. It adopts a forward approach and clearly it makes no use of target states, as there is no concept of target state in a feasible region.
Thus, it only explores the CMDPTS and collects states and actions that are feasibly reachable, provided the nature allows them to be chosen. The role of reload states is considered when updating the cost vector $\Vec{c}$. Nature here plays no role in identifying the feasible region; more precisely, nature can only prevent some state to be reached, but this does not affect whether such states or the other states are still potentially reachable in a feasible way}
\at{Explanation of Algorithm~\ref{alg:feasibleRegion}.
Data structures:
\begin{itemize}
\item
    $\Vec{c}(s)$: the minimum cost computed from the initial/state last reload state to reach $s$ through a feasible path ending in $s$
\item
    $\Vec{a}(s)$: actions from $s$ that we know will not make the cost exceed $\rcap$
\item
    $S_{f}$: set of states that are reachable through some feasible path
\item
    $\mathit{Queue}$: queue of states that need to be re-analyzed; if empty, it returns $\bot$
\item
    $s$: state currently under analysis that is feasibly reachable from the initial state
\item
    $c$: current minimal cost to reach $s$ from the beginning of the feasible path or the last reload state  
\end{itemize}
Behavior: 
\begin{itemize}
\item
    we start with the initial state ($s \gets \bar{s}$) as current state under analysis and since we are just at the beginning, we set $c \gets 0$. Note that we cannot set $\Vec{a}(\bar{s})$ to $0$ as this would affect other states reaching $\bar{s}$ later in the paths
\item
    we analyze $s$: we go over each action $a$ that does not make the cost $c + C(s, a)$ (current cost $c$ to have reached $s$ plus transition cost $C(s,a)$) exceed $\rcap$. For every possible successor $s'$, if the cost $c + C(s, a)$ is smaller than what we already know about it $\Vec{c}(s')$, we update its cost and enqueue it again for further analysis (why? Because the cost has been reduced, so some action might become feasible).
    Once done, we record that $a$ is feasible for $s$ ($\Vec{a}(s) \gets \Vec{a}(s) \cup \{a\}$).
\item
    once we have analyzed all actions, we record that $s$ is feasibly reachable ($S_{f} \gets S_{f} \cup \{s\}$) and then we take out the next state $s$ to analyze from the queue. If it is a reload state, we set its stored cost $\Vec{c}(s)$ to $0$ and set its current cost whatever is in $\Vec{c}(s)$ 
\end{itemize}
}
\at{Possible problems: the algorithm does not consider this case: $s_{0} \xrightarrow{a} s_{1} \xrightarrow{a} s_{2}$ and $s_{0} \xrightarrow{b} s_{1} \xrightarrow{b} s_{2}$ where the $a$-transitions cost 1 and the $b$-transitions 3; $\rcap = 4$. Of the possible paths, $s_{0} \{a,b\} s_{1} \{a,b\} s_{2}$, 3 are feasible and only $s_{0} b s_{1} b s_{2}$ is not. Still, $b$ will be in both $\Vec{a}(s_{0})$ and $\Vec{a}(s_{1})$. This is acceptable for feasibility checking and for space pruning. The synthesis algorithm needs to take care of this scenario.}
\begin{algorithm}
\caption{\proc{FeasibleRegion}}
\label{alg:feasibleRegion}
    \begin{algorithmic}[1]
        \Require CMDPST $\mdpst$
        \State initialize $\Vec{c} \in \naturals^{S}$ to be $\infty$ in every component
        \State initialize $\Vec{a} \in A^{S}$ to be $\emptyset$ in every component
        \State $S_{f} \gets \emptyset$; $\mathit{Queue} \gets \emptyset$; $s \gets \bar{s}$; $c \gets 0$
        \Repeat
            \ForAll{$a \in A(s)$ s.t. $c + C(s, a) \leq \rcap$}
                \ForAll{$s' \in \cup_{\Theta \in \mathcal{F}(s, a)} \Theta$}
                    \If{$\Vec{c}(s') > c + C(s,a)$}
                        \State $\Vec{c}(s') = c + C(s, a)$
                        \State $\mathit{Queue}.\mathit{enqueue}(s')$
                    \EndIf
                \EndFor
                \State $\Vec{a}(s) \gets \Vec{a}(s) \cup \{a\}$
            \EndFor
            \State $S_{f} \gets S_{f} \cup \{s\}$
            \State $s \gets \mathit{Queue}.\mathit{dequeue}$
            \If{$s \in R$} 
                $\Vec{c}(s) \gets 0$
            \EndIf
            \State $c \gets \Vec{c}(s)$
        \Until{$s \neq \bot$}
        \State \Return $S_{f}, \Vec{a}$
    \end{algorithmic}
\end{algorithm}


==> sections/computer_winning_region_alt.tex <==
\section{Optimal Robust Strategy Synthesis}
\label{sec:strategySynthesis}

\at{In what follows, I assume that it is possible to have $\Theta \in \mathcal{F}(s, a)$ but $\mathcal{T}(s, a, \Theta) = 0$ or undefined. I don't like this situation (as I find it not so reasonable), but this is what we have from the current definitions\dots}

\at{This paragraph seems not so connected with the actual material introduced in the section}
To enable high-level task planning for systems with \textbf{resource constraints} and \textbf{unquantifiable uncertainty}, we introduce \textit{Linear Temporal Logic over finite traces} ($\ltlf$) into the framework of MDPST.
Unlike classical $\ltl$, which is interpreted over infinite traces, $\ltlf$ is interpreted over finite trajectories, making it particularly suitable for specifying \textbf{one-shot reachability goals}--that is, whether the system can reach a target state from the initial state under resource limitations.

Building upon this specification framework, we formulate the \textbf{Optimal Robust Strategy Synthesis} problem.
Given a CMDPST model $\mdpst$ and an $\ltlf$ specification $\varphi$, the objective is to synthesize a strategy such that, under all possible unquantifiable uncertainties (i.e., adversarial nature), the agent maximizes the probability of satisfying the high-level task described by $\varphi$.

\at{Before going into the technical details, it is better to provide an informal overview of the steps leading to the solution of the problem. Right now things are introduced but it is not clear why they are needed and for what they actually used for.}
\py{Agree. In addition, in the above problem description, we need to mention the consumption constraints.  }

\subsection{Construct product CMDPST}

\at{I now propose a new construction, where failure states are explicitly constructed. Also note the change in the $\ltlf$ formula}
\begin{definition}[Product CMDPST]
    Given a CMDPST $\mdpst = (S, \bar{s}, A, \mathcal{F}, \mathcal{T}, L, C, R, \rcap)$ and an $\ltlf$ formula $\varphi$ over $\AP$, let $\exhausted$ be a fresh atomic proposition, $\psi = \varphi \land \lglobally \neg \exhausted$, and $\dfa_{\psi} = (2^{\AP \cup \{\exhausted\}}, Q, \bar{q}, \delta, \acc)$ be its corresponding DFA. 

    The \emph{product CMDPST} is defined as:
    \[
        \mdpst^{\times} = (S^{\times}, \bar{s}^{\times}, A^{\times}, \mathcal{F}^{\times}, \mathcal{T}^{\times}, L^{\times}, C^{\times}, R^{\times}, \rcap^{\times}, \mathsf{Acc}^{\times})
    \]
    with the following components:
    \begin{itemize}
    \item 
        $S^{\times} \subseteq S \times Q \times ([0, \rcap] \cup \{\exhausted\})$ is the smallest set such that $(\bar{s}, \bar{q}, \rcap) \in S^{\times}$ and is closed under the functions $\mathcal{F}^{\times}$ and $\mathcal{T}^{\times}$ defined below.
        States $(s, q, c)$ and $(s, q, \exhausted)$ encode the system state $s$, the DFA state $q$, and the remaining resource $c \in [0, \rcap]$ or resources being exhausted, respectively. 
    \item 
        $\bar{s}^{\times} = (\bar{s}, \bar{q}, \rcap)$.
    \item 
        $A^{\times} = A$.
    \item 
        $L^{\times}((s, q, c)) = L(s)$ and $L^{\times}((s, q, \exhausted)) = L(s) \cup \{\exhausted\}$.
    \item 
        $\mathcal{F}$ and $\mathcal{T}$ are constructed as follows:
        \begin{itemize}
        \item 
            for $(s, q, c) \in S^{\times}$ and $a \in A(s)$ such that $C(s, a) \leq c$:
            \begin{itemize}
            \item 
                Compute the DFA successor state $q' = \delta(q, L(s))$.
            \item 
                For each $\Theta \in \mathcal{F}(s, a)$:
                construct the transition set
                \begin{align*}
                    \Theta^{\times} & = \setcond{(s', q', \rcap)}{s' \in \Theta \cap R} \cup {}\\
                    & \hphantom{{} = {}} \setcond{(s', q', c - C(s, a))}{s' \in \Theta \setminus R};
                \end{align*}
                if $\Theta^{\times} \neq \emptyset$, then add $\mathcal{F}^{\times}((s, q, c), a) \ni \Theta^{\times}$ and set $\mathcal{T}^{\times}((s, q, c), a, \Theta^{\times}) = \mathcal{T}(s, a, \Theta)$.
            \end{itemize}
        \item
            for $(s, q, c) \in S^{\times}$ and $a \in A(s)$ such that $C(s, a) > c$:
            set $\mathcal{F}^{\times}((s, q, c), a) = \{(s, q, \exhausted)\}$ and set $\mathcal{T}^{\times}((s, q, c), a, \{(s, q, \exhausted)\}) = 1$.
        \item
            for $(s, q, \exhausted) \in S^{\times}$ and $a \in A(s)$:
            $\mathcal{F}^{\times}((s, q, \exhausted), a) = \{(s, q, \exhausted)\}$ and $\mathcal{T}^{\times}((s, q, \exhausted), a, \{(s, q, \exhausted)\}) = 1$.            
        \end{itemize}
    \item 
        $C^{\times}((s, q, c), a) = C(s, a)$ and $C^{\times}((s, q, \exhausted), a) = 0$.
    \item 
        $R^{\times} = \setcond{(s, q, c) \in S^{\times}}{s \in R}$.
    \item 
        $\rcap^{\times} = \rcap$.
    \item 
        $\acc^{\times} = \setcond{(s, q, c) \in S^{\times}}{q \in \acc}$.
    \end{itemize}
\end{definition}

This construction enables synchronized progression of the system and the $\ltlf$ specification while tracking resource availability, forming the basis for robust reachability and optimal strategy synthesis in subsequent sections.
States $(s, q, \exhausted)$ represent \emph{exhausted} states, meaning that the system has run out of resources, so it is stuck in them.
The $\ltlf$ formula $\psi = \varphi \land \lglobally \neg \exhausted$ holds for the paths that satisfy $\varphi$ and never enter an exhausted state;
by construction, this ensures that the system never exceeds the resource constraints.





\subsection{Computing the winning region}
After constructing the product CMDPST $\mdpst^{\times}$, the central problem we aim to solve is the following: 
\emph{Does there exist a strategy that, starting from the initial state $\bar{s}^{\times}$, can safely reach the set of target states $\acc^{\times}$ under resource constraints and adversarial transition behaviors, thereby satisfying the $\ltlf$ specification $\varphi$?}

Due to limited resource capacity and the uncertainty in the set-valued transitions, we cannot rely on classical MDP planning techniques that assume expected value updates or fixed probabilistic dynamics.
Instead, we must ensure that the synthesized strategy remains valid under all possible resolutions of set-valued transitions.
To address this challenge, we introduce the concept of the \emph{winning region}, which characterizes the set of states that can contribute to the satisfaction of the task under some feasible strategy.

\begin{definition}[Winning region]
\label{def:winningRegion}
    Given a product CMDPST $\mdpst^{\times}$, the \emph{winning region} $W \subseteq S^{\times}$ is the set of states that satisfy the following two conditions:
    % \begin{itemize}
    % \item
        $\acc^{\times} \subseteq W$ and
    % \item
        % for each $s \in W$, there is $a \in A^{\times}(s)$ such that for all $\mathfrak{h}^{a}_{s} \in \mathfrak{H}^{a}_{s}$, $\mathfrak{h}^{a}_{s}(W) = 1$.
    % \item 
        for each $s \in W$, there is $a \in A^{\times}$ such that for all $\Theta \in \mathcal{F}^{\times}(s, a)$, if $\mathcal{T}^{\times}(s, a, \Theta) > 0$ then $\Theta \subseteq W$.
    % \end{itemize}
    \at{Note that by construction of $\mdpst^{\times}$, all states in $S^{\times}$ and $\acc^{\times}$ are potentially reachable (so the winning region is also potentially reachable), but there is no guarantee that they are actually reachable as this depends on the feasible distribution chosen by nature}
    \end{definition}

The above definition of winning region directly provides us with an algorithm for obtaining it:
we need to compute the least fixed-point of the function 
$\mathit{wr}(W) = W \cup \setcond{s \in S^{\times}}{\exists a \in A^{\times}. \forall \Theta \in \mathcal{F}^{\times}(s, a). \mathcal{T}^{\times}(s, a, \Theta) > 0 \implies \Theta \subseteq W}$ starting from $\mathit{wr}(\acc^{\times})$.






\subsection{Synthesize and Extract the Optimal Robust Strategy}

Based on the constructed product CMDPST $\mdpst^{\times}$ and the identified winning region $W$, we now focus on synthesizing an optimal strategy that guarantees the satisfaction of the $\ltlf$ specification $\varphi$ under worst-case transition behaviors.
Since the specification is defined over finite traces, the strategy synthesis problem reduces to computing a policy that maximizes the probability of reaching the winning region $W$ from the initial state $\bar{s}^{\times}$.


\begin{definition} 
\label{def:robustValueFunction}
    Given the product CMDPST $\mdpst^{\times} = (S^{\times}, \bar{s}^{\times}, A^{\times}, \mathcal{F}^{\times}, \mathcal{T}^{\times}, L^{\times}, C^{\times}, R^{\times}, \rcap^{\times}, \acc^{\times})$ and a winning region $W \subseteq S^{\times}$, the \emph{robust value function} $V \colon S^{\times} \to [0,1]$ is defined as:
    \[
        V(s) = \max_{\strategy \in \strategies_{\mdpst^{\times}}} \min_{\nature \in \natures_{\mdpst^{\times}}} \prob^{\strategy, \nature}_{s}(\lfinally W)
    \]
    where $\strategy$ is the agent’s strategy and $\nature$ is the nature’s strategy (resolving nondeterminism). 
    For all $s \in W$, we set $V(s) = 1$. 
    For $s \in S^{\times} \setminus W$, $V(s)$ satisfies the following \emph{robust Bellman equation}:
    \at{This definition looks wrong to me: in my opinion, it should have $\min_{\mathfrak{h}^{a}_{s} \in \mathfrak{H}^{a}_{s}} \sum_{s' \in \Theta} \mathfrak{h}^{a}_{s}(s') \cdot V(s')$ (or, more correctly, $\inf$) instead of $\min_{s' \in \Theta} V(s')$}
    \at{The definition below would match the proposed change if we allow nature to disable successor states, e.g., for $\Theta = \{s_0, s_1\} \in \mathcal{F}(s,a)$, we allow nature to induce the feasible distribution $\mathfrak{h}^{a}_{s}$ such that $\mathfrak{h}^{a}_{s}(s_{0}) = 1$ and $\mathfrak{h}^{a}_{s}(s_{1}) = 0$. Then clearly such point distributions are always available for each $\Theta$ and thus nature can just lead to the state with lowest value. However, if we allow this freedom to nature, then one might wonder why we need to use feasible distribution\dots}
    \[
        V(s) = \max_{a \in A(s)} \sum_{\Theta \in \mathcal{F}^{\times}(s,a)} \mathcal{T}^{\times}(s, a, \Theta) \cdot \min_{s' \in \Theta} V(s')
    \]
    \end{definition}
This definition captures the worst-case reachability probability under both adversarial nondeterminism and probabilistic uncertainty.
This operator reflects the trade-off between strategic choice (max over actions) and worst-case behavior of nature (min over successor states in each $\Theta$).
Finally, after obtaining the optimal robust strategy, we map it back to the original CMDPST to derive an executable control policy.

\at{We do not provide a specific algorithm for doing so and we do not say how it can be intuitively done, do we? Also, when we map back, do we still have stationary strategies or do we need history-dependent strategies as it happens for ordinary MDPs against $\ltl$?}


==> sections/computer_winning_region_ms.tex <==
\section{Optimal Robust Strategy Synthesis}
\label{sec:strategySynthesis}

\at{This is a version where we first restrict the CMDPST to have only resource constrained paths; then we make the product with the DFA}

\at{In what follows, I assume that it is possible to have $\Theta \in \mathcal{F}(s, a)$ but $\mathcal{T}(s, a, \Theta) = 0$ or undefined. I don't like this situation (as I find it not so reasonable), but this is what we have from the current definitions\dots}

\at{Before going into the technical details, it is better to provide an informal overview of the steps leading to the solution of the problem. Right now things are introduced but it is not clear why they are needed and for what they actually used for.}
\py{Agree. In addition, in the above problem description, we need to mention the consumption constraints.  }


\subsection{Resource constrained CMDPST}



\begin{definition}[Resource constrained CMDPST]
    Given a CMDPST $\mdpst = (S, \bar{s}, A, \mathcal{F}, \mathcal{T}, L, C, R, \rcap)$, let $\exhausted$ be a fresh atomic proposition. 
    The \emph{resource constrained CMDPST} (RCMDPST) $\mdpst^{\exhausted}$ is defined as:
    \[
        \mdpst^{\exhausted} = (S^{\exhausted}, \bar{s}^{\exhausted}, A^{\exhausted}, \mathcal{F}^{\exhausted}, \mathcal{T}^{\exhausted}, L^{\exhausted}, C^{\exhausted}, R^{\exhausted}, \rcap^{\exhausted})
    \]
    with the following components:
    \begin{itemize}
    \item 
        $S^{\exhausted} \subseteq (S \times [0, \rcap]) \cup (S \times \{\exhausted\})$ is the smallest set such that $(\bar{s}, \rcap) \in S^{\exhausted}$ that is closed under the functions $\mathcal{F}^{\exhausted}$ and $\mathcal{T}^{\exhausted}$ defined below.
        A state $(s, r) \in S^{\exhausted}$ is either a states $(s, c) \in S \times [0, \rcap]$ or a $(s, \exhausted) \in S \times \{\exhausted\}$ encoding the CMDPST state $s$ and the remaining resource $r = c \in [0, \rcap]$ or resources being exhausted ($r = \exhausted$), respectively. 
    \item 
        $\bar{s}^{\exhausted} = (\bar{s}, \rcap)$.
    \item 
        $A^{\exhausted}((s, r)) = A(s)$ for all $(s, r) \in S^{\exhausted}$.
    \item 
        $L^{\exhausted}((s, c)) = L(s)$ and $L^{\exhausted}((s, \exhausted)) = L(s) \cup \{\exhausted\}$ for all $(s, c), (s, \exhausted) \in S^{\exhausted}$.
    \item 
        $\mathcal{F}^{\exhausted}$ and $\mathcal{T}^{\exhausted}$ are constructed as follows:
        \begin{itemize}
        \item 
            for all $(s, c) \in S^{\exhausted}$ and $a \in A(s)$ such that $C(s, a) \leq c$ and for each $\Theta \in \mathcal{F}(s, a)$, let
            $\Theta^{\exhausted} = \setcond{(s', \rcap)}{s' \in \Theta \cap R} \cup \setcond{(s', c - C(s, a))}{s' \in \Theta \setminus R}$;
%             \begin{align*}
%                 \Theta^{\exhausted} & = \setcond{(s', \rcap)}{s' \in \Theta \cap R} \cup {}\\
%                 & \hphantom{{} = {}} \setcond{(s', c - C(s, a))}{s' \in \Theta \setminus R};
%             \end{align*}
            then add $\mathcal{F}^{\exhausted}((s, c), a) \ni \Theta^{\exhausted}$ and set $\mathcal{T}^{\exhausted}((s, c), a, \Theta^{\exhausted}) = \mathcal{T}(s, a, \Theta)$.
        \item
            for all $(s, c) \in S^{\exhausted}$ and $a \in A(s)$ such that $C(s, a) > c$:
            set $\mathcal{F}^{\exhausted}((s, c), a) = \{(s, \exhausted)\}$ and $\mathcal{T}^{\exhausted}((s, c), a, \{(s, \exhausted)\}) = 1$.
        \item
            for all $(s, \exhausted) \in S^{\exhausted}$ and $a \in A(s)$:
            set $\mathcal{F}^{\exhausted}((s, \exhausted), a) = \{(s, \exhausted)\}$ and $\mathcal{T}^{\exhausted}((s, \exhausted), a, \{(s, \exhausted)\}) = 1$.            
        \end{itemize}
    \item 
        $C^{\exhausted}((s, c), a) = C(s, a)$ and $C^{\exhausted}((s, \exhausted), a) = 0$ for all $(s, c), (s, \exhausted) \in S^{\exhausted}$.
    \item 
        $R^{\exhausted} = \setcond{(s, r) \in S^{\exhausted}}{s \in R \land r \neq \exhausted}$.
    \item 
        $\rcap^{\exhausted} = \rcap$.
    \end{itemize}
\end{definition}
States $(s, \exhausted)$ represent \emph{exhausted} states, meaning that the system has run out of resources, so it is stuck in them.
When the system tries to perform an action $a$ from a state $(s, c)$ with $C(s, a) > c$, the system exhausts its resources and fails to perform the action; 
this is modeled by forcing the system to transition from state $(s, c)$ to $(s, \exhausted)$.



\subsection{Construct product CMDPST}

\begin{definition}[Product CMDPST]
    Given an RCMDPST $\mdpst = (S^{\exhausted}, \bar{s}^{\exhausted}, A^{\exhausted}, \mathcal{F}^{\exhausted}, \mathcal{T}^{\exhausted}, L^{\exhausted}, C^{\exhausted}, R^{\exhausted}, \rcap^{\exhausted})$ and an $\ltlf$ formula $\varphi$ over $\AP$, let $\dfa_{\varphi} = (\Sigma, Q, \bar{q}, \delta, \acc)$ be its corresponding DFA. 
    The \emph{product RCMDPST} $\mdpst^{\times}$ is defined as:
    \[
        \mdpst^{\times} = (S^{\times}, \bar{s}^{\times}, A^{\times}, \mathcal{F}^{\times}, \mathcal{T}^{\times}, L^{\times}, C^{\times}, R^{\times}, \rcap^{\times}, \mathsf{Acc}^{\times})
    \]
    with the following components:
    \begin{itemize}
    \item 
        $S^{\times} \subseteq S^{\exhausted} \times Q$ is the smallest set such that $(\bar{s}^{\exhausted}, \bar{q}) \in S^{\times}$ and is closed under the functions $\mathcal{F}^{\times}$ and $\mathcal{T}^{\times}$ defined below.
    \item 
        $\bar{s}^{\times} = (\bar{s}^{\exhausted}, \bar{q})$.
    \item 
        $A^{\times}((s^{\exhausted}, q)) = A^{\exhausted}(s^{\exhausted})$ for all $(s^{\exhausted}, q) \in S^{\times}$.
    \item 
        $L^{\times}((s^{\exhausted}, q)) = L(s^{\exhausted})$ for all $(s^{\exhausted}, q) \in S^{\times}$.
    \item 
        $\mathcal{F}^{\times}$ and $\mathcal{T}^{\times}$ are constructed as follows:
        for each $(s^{\exhausted}, q) \in S^{\times}$ and $a^{\exhausted} \in A(s^{\exhausted})$, let $\Theta'$ denote the set $\Theta \times \{\delta(q, L(s^{\exhausted}))\}$, where $\Theta \in \mathcal{F}^{\exhausted}(s^{\exhausted}, a^{\exhausted})$.
        Then, define $\mathcal{F}^{\times}((s^{\exhausted}, q), a^{\exhausted}) = \setcond{\Theta'}{\Theta \in \mathcal{F}^{\exhausted}(s^{\exhausted}, a^{\exhausted})}$ and $\mathcal{T}^{\times}((s^{\exhausted}, q), a^{\exhausted}, \Theta') = \mathcal{T}^{\exhausted}(s^{\exhausted}, a^{\exhausted}, \Theta)$ for each $\Theta \in \mathcal{F}^{\exhausted}(s^{\exhausted}, a^{\exhausted})$.
    \item 
        $C^{\times}((s^{\exhausted}, q), a) = C(s^{\exhausted}, a)$ for all $(s^{\exhausted}, q) \in S^{\times}$ and $a^{\exhausted} \in A^{\times}((s^{\exhausted}, q))$.
    \item 
        $R^{\times} = \setcond{(s^{\exhausted}, q) \in S^{\times}}{s^{\exhausted} \in R^{\exhausted}}$.
    \item 
        $\rcap^{\times} = \rcap^{\exhausted}$.
    \item 
        $\acc^{\times} = \setcond{(s^{\exhausted}, q) \in S^{\times}}{\exhausted \notin L^{\exhausted}(s^{\exhausted}) \land q \in \acc}$.
    \end{itemize}
\end{definition}

This construction enables synchronized progression of the system and the $\ltlf$ specification while tracking resource availability, forming the basis for robust reachability and optimal strategy synthesis in subsequent sections.

\at{Since exhausted states are never going to be accepting, we can directly remove all of them before performing robust strategy synthesis, as anyway they do not contribute to maximizing the winning probability.}



\subsection{Computing the winning region}
After constructing the product CMDPST $\mdpst^{\times}$, the central problem we aim to solve is the following: 
\emph{Does there exist a strategy that, starting from the initial state $\bar{s}^{\times}$, can safely reach the set of target states $\acc^{\times}$ under resource constraints and adversarial transition behaviors, thereby satisfying the $\ltlf$ specification $\varphi$?}

Due to limited resource capacity and the uncertainty in the set-valued transitions, we cannot rely on classical MDP planning techniques that assume expected value updates or fixed probabilistic dynamics.
Instead, we must ensure that the synthesized strategy remains valid under all possible resolutions of set-valued transitions.
To address this challenge, we introduce the concept of the \emph{winning region}, which characterizes the set of states that can contribute to the satisfaction of the task under some feasible strategy.

\begin{definition}[Winning region]
\label{def:winningRegion}
    Given a product CMDPST $\mdpst^{\times}$, the \emph{winning region} $W \subseteq S^{\times}$ is the set of states that satisfy the following two conditions:
    % \begin{itemize}
    % \item
        $\acc^{\times} \subseteq W$ and
    % \item
        % for each $s \in W$, there is $a \in A^{\times}(s)$ such that for all $\mathfrak{h}^{a}_{s} \in \mathfrak{H}^{a}_{s}$, $\mathfrak{h}^{a}_{s}(W) = 1$.
    % \item 
        for each $s \in W$, there is $a \in A^{\times}$ such that for all $\Theta \in \mathcal{F}^{\times}(s, a)$, if $\mathcal{T}^{\times}(s, a, \Theta) > 0$ then $\Theta \subseteq W$.
    % \end{itemize}
    \at{Note that by construction of $\mdpst^{\times}$, all states in $S^{\times}$ and $\acc^{\times}$ are potentially reachable (so the winning region is also potentially reachable), but there is no guarantee that they are actually reachable as this depends on the feasible distribution chosen by nature}
    \end{definition}

The above definition of winning region directly provides us with an algorithm for obtaining it:
we need to compute the least fixed-point of the function 
$\mathit{wr}(W) = W \cup \setcond{s \in S^{\times}}{\exists a \in A^{\times}. \forall \Theta \in \mathcal{F}^{\times}(s, a). \mathcal{T}^{\times}(s, a, \Theta) > 0 \implies \Theta \subseteq W}$ starting from $\mathit{wr}(\acc^{\times})$.






\subsection{Synthesize and Extract the Optimal Robust Strategy}

Based on the constructed product CMDPST $\mdpst^{\times}$ and the identified winning region $W$, we now focus on synthesizing an optimal strategy that guarantees the satisfaction of the $\ltlf$ specification $\varphi$ under worst-case transition behaviors.
Since the specification is defined over finite traces, the strategy synthesis problem reduces to computing a policy that maximizes the probability of reaching the winning region $W$ from the initial state $\bar{s}^{\times}$.


\begin{definition} 
\label{def:robustValueFunction}
    Given the product CMDPST $\mdpst^{\times} = (S^{\times}, \bar{s}^{\times}, A^{\times}, \mathcal{F}^{\times}, \mathcal{T}^{\times}, L^{\times}, C^{\times}, R^{\times}, \rcap^{\times}, \acc^{\times})$ and a winning region $W \subseteq S^{\times}$, the \emph{robust value function} $V \colon S^{\times} \to [0,1]$ is defined as:
    \[
        V(s) = \max_{\strategy \in \strategies_{\mdpst^{\times}}} \min_{\nature \in \natures_{\mdpst^{\times}}} \prob^{\strategy, \nature}_{s}(\lfinally W)
    \]
    where $\strategy$ is the agent’s strategy and $\nature$ is the nature’s strategy (resolving nondeterminism). 
    For all $s \in W$, we set $V(s) = 1$. 
    For $s \in S^{\times} \setminus W$, $V(s)$ satisfies the following \emph{robust Bellman equation}:
    \[
        V(s) = \max_{a \in A(s)} \sum_{\Theta \in \mathcal{F}^{\times}(s,a)} \mathcal{T}^{\times}(s, a, \Theta) \cdot V_{\inf}(s, a, \Theta),
    \]
    where $V_{\inf}(s, a, \Theta) = \inf_{\mathfrak{h}^{a}_{s} \in \mathfrak{H}^{a}_{s}} \sum_{s' \in \Theta} \mathfrak{h}^{a}_{s}(s') \cdot V(s')$.
    \end{definition}
This definition captures the worst-case reachability probability under both adversarial nondeterminism and probabilistic uncertainty.
This operator reflects the trade-off between strategic choice (max over actions) and worst-case behavior of nature (min over successor states in each $\Theta$).
Finally, after obtaining the optimal robust strategy, we map it back to the original CMDPST to derive an executable control policy.

\at{We do not provide a specific algorithm for doing so and we do not say how it can be intuitively done, do we? Also, when we map back, do we still have stationary strategies or do we need history-dependent strategies as it happens for ordinary MDPs against $\ltl$?}


==> sections/maximize_LTLf_satisfying_probability.tex <==
\section{Maximize Satisfying Probability under Resource Constraints}
\label{Maximize Satisfying Probability}

\py{Let me clarify here. At the end of Section 4, we've computed the maximum probability of satisfying the given $\ltlf$ specification while ensuring that resources are not exhausted during execution, right?}

In this section, we aim to maximize the probability of satisfying the given $\ltlf$ specification while ensuring that resources are not exhausted during execution. 
To achieve this, we incorporate resource constraints into the $\ltlf$ formulation to guarantee resource availability throughout the task.

Following the approach in Section~\ref{sec:strategySynthesis}, we incorporate the $\ltlf$ formula into the original consumption CMDPST by constructing a product CMDPST $\mdpst^{\times}$. 
Based on this construction, we identify the winning region $W$ consisting of:
\at{Target states are now the accepting states $\acc^{\times}$, right?}
\yh{i think so}
\begin{itemize}
    \item target states that are reachable from the initial state even under the worst-case transition choices;
    \item and reload states that are reachable from the initial state and from which some target state is also reachable under worst-case transitions.
\end{itemize}

Next, we proceed to synthesize a strategy that guarantees resource availability throughout the execution while maximizing the probability of reaching the winning region $W$.

\at{Below, is the "sub" subscript really needed? Can't we just use $\mdpst^{\times}$ instead of $\mdpst_{\text{sub}}^{\times}$? Otherwise we should explain what "sub" stands for. Similarly for the "pre" subscript}
\yh{We use sub because we have replaced ACC with W. Perhaps pre can be removed?}
\at{Nowhere it is written that $\mdpst_{\text{sub}}^{\times}$ is $\mdpst^{\times}$ with $\acc^{\times}$ replaced by $W$. This has to be made clear and probably it is better to write $\mdpst^{\times}_{W}$ instead}
Given an infinite path $\xi^{\times} = s_{0}^{\times} a_{0}^{\times} s_{1}^{\times} a_{1}^{\times} \cdots$ of the product CMDPST $\mdpst_{\text{sub}}^{\times}$, and a designated winning region $W$, we define the total cost of the path as:
\[
    \cost_{\text{pre}}(\xi^{\times}) = \sum_{t=0}^{T-1} C^{\times}(s_{t}^{\times}, a_{t}^{\times})
\]
where $T = \argmin_{t} \{ s_{t}^{\times} \in W \}$ is the first time the path reaches $W$ and we consider a path $\xi^{\times}$ to be \emph{resource-safe} if the available resource is never exhausted before reaching $W$. 
Formally, we require:
\[
    \forall t < T.\quad \sum_{\tau=0}^{t} C^{\times}(s_{\tau}^{\times}, a_{\tau}^{\times}) < \rcap.
\]
Let $\Xi_{\text{safe}}$ denote the set of all such resource-safe paths.

Given the initial state $\bar{s}^{\times}$ and a strategy $\strategy^{\times}$, the probability of eventually and safely reaching $W$ is defined as:
\[
P_{\text{safe}}(\bar{s}^{\times}, W, \strategy^{\times}) := 
\prob_{\mdpst_{\text{sub}}^{\times}}^{\strategy^{\times}}
\left( \text{$\Xi_{\text{safe}}$ and $\lfinally W$} \right)
\]

\at{Finite execution paths are also affected by nature}
Let $\fpaths^{\strategy^{\times}}(\bar{s}^{\times})$ denote the set of all finite execution paths generated under strategy $\strategy^{\times}$ starting from the initial state $\bar{s}^{\times}$. 
We define the problem as follows:
%\at{The problem below ignores that $\xi^{\times}$ can pass through a reload state. Moreover, the product construction already ensures that $\rcap$ is never exceeded (by taking into account also the effect of the reload states) }
%\yh{i think we previously extracted the effective reload states and incorporated them into the winning region. We ignore the effects of all other reload states. The product structure ensures that the states within the winning region are reachable from the initial state (strategically reachable, meaning there exists a strategy to reach them), but it does not guarantee that all actions are reachable. Our approach here is first to extract the winning region consisting of states reachable from the initial state. Then, we eliminate actions that would cause resource exhaustion or negative resources during the process. This ensures that the remaining actions will not lead to resource exhaustion at any intermediate step.}
%\at{Still, the definition of the problem ignores the contribution of the reload states: it just says that the overall cost along the path is below $\rcap$; whether a reload state is visited or not does not affect the sum. This means, for instance, that if each transition costs $1$ and $\rcap$ is set to $5$, all paths of length 5 or more that reach the winning region are excluded, even if they only visit reload states. Do we really want this?}
%\yh{I think that the remaining reload states we ultimately have are the Rvalid filtered by Algorithm 3. In other words, the remaining reload states must be reachable from the initial state in the worst-case scenario and also able to reach the goal state. The other reload states are completely meaningless because reaching or passing through them would lead to resource exhaustion midway. Therefore, we cannot pass through them. Since Rvalid has already been incorporated into the Winning region, the other reload states can be completely ignored. I wonder if my understanding is correct}
\begin{problem}
Given the product CMDPST $\mdpst_{\text{sub}}^{\times}$, compute an optimal stationary strategy $\strategy_{\text{pre}}^{*} \in \Pi^{\times}$ such that:
\[
    \max_{\strategy^{\times} \in \Pi^{\times}} \quad \prob^{\strategy^{\times}}(\lfinally W)
\]
subject to:
\[
\forall \xi^{\times} \in \fpaths^{\strategy^{\times}}(\bar{s}^{\times}). \forall t < T_{\xi^{\times}}. \sum_{\tau=0}^{t} C^{\times}(s_{\tau}^{\times}, a_{\tau}^{\times}) < \rcap.
\]
\end{problem}

That is, we seek to maximize the probability of eventually reaching the winning region $W$, under the hard constraint that the system never exhausts its resources along any path before reaching $W$.

To solve the constrained probability maximization problem described above, we propose the following four-step approach:

\begin{enumerate}
    \item We transform the original finite-horizon resource-constrained optimization problem into an equivalent infinite-horizon formulation.
    
    \item We prune all unsafe transitions that may lead to resource exhaustion, resulting in a resource-safe product MDPST.
    
    \item We present an algorithm to approximate the optimal stationary strategy over this resource-safe model.
\end{enumerate}







\subsection{Horizon Extension}
\label{Horizon Extension}

Given the product CMDPST $\mdpst_{\text{sub}}^{\times}$ and the winning accepting region $W$, we start by defining a modified CMDPST $\mdpst[Z]_{\text{pre}}$ of $\mdpst_{\text{sub}}^{\times}$ as
\[
    \mdpst[Z]_{\text{pre}} = (S_{\text{pre}}, \bar{s}^{\times}, A_{\text{pre}}, \mathcal{F}_{\text{pre}}, \mathcal{T}_{\text{pre}}, L^{\times}, C_{\text{pre}}, R_{\text{pre}}, \rcap^{\times}, W),
\]
where 
% $S_{\text{pre}} = S^{\times} \setminus \setcond{s^{\times} \in \acc^{\times}}{s^{\times} \notin W^{\times}}$ and 
$S_{\text{pre}} = S^{\times} \setminus (\acc^{\times} \setminus W)$ and 
$A_{\text{pre}} = A^{\times} \cup \{\tau\}$ with $\tau$ being a fresh action. 
%
The set-valued transition function $\mathcal{F}_{\text{pre}}$ is defined as follows: 
\at{Adding a clarification about enabled actions}
i) for all $s^{\times} \in  W^{\times}$, $A_{\text{pre}}(s^{\times}) = \{\tau\}$ and $\mathcal{F}_{\text{pre}}(s^{\times}, \tau) = \{\{s^{\times}\}\}$, and 
ii) for all $s^{\times} \in  S_{\text{pre}} \setminus W$, $A_{\text{pre}}(s^{\times}) = A^{\times}(s^{\times})$ and $\Theta \in \mathcal{F}_{\text{pre}}(s^{\times}, a^{\times})$ iff $\Theta \in \mathcal{F}_{p}(s^{\times}, a^{\times})$ and $\Theta \subseteq S_{\text{pre}}$. 
%
The transition probability function is given by:
\at{Adding missing case for self-loops}
i) for all $s^{\times} \in  W^{\times}$, $\mathcal{T}_{\text{pre}}(s^{\times}, \tau, \{s^{\times}\}) = 1$, and 

%\at{What is $\mathcal{T}_{p}$? I presume it is $\mathcal{T}^{\times}$, right?}
ii) for all $s^{\times} \in  S_{\text{pre}} \setminus W$, $\mathcal{T}_{\text{pre}}(s^{\times}, a^{\times}, \Theta) = \mathcal{T}^{\times}(s^{\times}, a^{\times}, \Theta)$. 
%\at{What is $S_{\text{acc}}$? I presume it is $W$, right?}
Finally, the cost function $C_{\text{pre}}$ is defined by 
$C_{\text{pre}}(s^{\times}, a^{\times}) = C^{\times}(s^{\times}, a^{\times})$ for all $s \in  S_{\text{pre}} \setminus W^{\times}$ and 
$C_{\text{pre}}(s, \tau) = 0$ for all $s \in W^{\times}$.
\at{$R_{\text{pre}}$ is not defined. I presume it is $R_{\text{pre}} = R^{\times} \cap S_{\text{pre}}$, right?}

The infinite-horizon total cost function $\cost_{\text{pre}}$ for an infinite path $\fpath^{\times}h$ of $\mdpst[Z]_{\text{pre}}$ is given by
\[\cost_{\text{pre}}(\fpath^{\times}) = \sum_{t=0}^\infty C_{\text{pre}}(s_{t}^{\times}, a_{t}^{\times}).\] 
Then the expected total cost induced by $\strategy^{\times}$ of $\mdpst[Z]_{\text{pre}}$ is given by
\at{where is nature here?}
\[\hat{Q}_{\text{pre}}(\bar{s}^{\times}, \sigma^{\times}) := \text{Exp}_{\xi^{\times} \in \hat{\Omega}^{\sigma^{\times}}(\bar{s}^{\times})}[\text{Cost}_{\text{pre}}(\xi^{\times})],\]
where $\hat{\Omega}^{\sigma^{\times}}(\bar{s}^{\times})$ is the set of all infinite paths of $Z_{\text{pre}}$ generated by $\sigma^{\times}$ from $\bar{s}^{\times}$.

It's straightforward to show that
%\at{$Q_{\text{pre}}(\bar{s}^{\times},S_{\text{acc}}, \sigma^{\times})$ is not defined}
\[\hat{Q}_{\text{pre}}(\bar{s}^{\times},\sigma^{\times})=\mathbb{E}^{\sigma^{\times}}_{\bar{s}^{\times}} \left[ \sum_{t=0}^{T - 1} C_{\text{pre}}(s_t^{\times}, a_t^{\times}) \right]\]
where $T$ is the first time $s_T^{\times} \in W$
since the cost of staying in $W$ is zero in $\mdpst[Z]_{\text{pre}}$.









\subsection{Safety Pruning}

To ensure that the synthesized strategy will never lead to resource exhaustion before reaching the target, we conservatively remove all actions that may result in unsafe transitions. 

Given a state $s \in S$ and action $a \in A(s)$, we define the pessimistic total cost of executing action $a$ from state $s$ as:
%\at{What is $\text{TotalCost}(s,a)$?}
\[
x(s) := \max_{\substack{a \in A(s) \\ \text{TotalCost}(s,a) < \infty}} 
\Big( C(s,a) + \max_{\Theta \in \mathcal{F}(s,a)} \max_{s' \in \Theta} x(s') \Big)
\]


% $C(s,a)$ denotes the immediate resource cost of executing action $a$ at state $s$, and $\mathcal{F}(s,a)$ is the nondeterministic transition function mapping a state-action pair to a set of possible successor sets. 
Here, $\text{TotalCost}(s,a)$ is the worst-case accumulated cost along all possible paths starting from $s$ with initial action $a$ under the given transition structure. We assume actions leading to infinite cost are excluded from consideration. The outer max over actions selects the worst-case action $a$ among all executable actions at $s$ whose total cost is finite. 
This models a conservative controller that assumes the maximal cost valid action will be taken. 
The maximization over $\Theta \in \mathcal{F}(s,a)$ and $s' \in \Theta$ models the worst-case environment choice.



We define the safety of actions based on the pessimistic cost value $x(s)$ and the capacity limit $\rcap$. 
\begin{definition}
\label{safety definition}
Given the pessimistic cost function $x(s)$ and the resource capacity bound $\rcap$, we define the \emph{safe action set} for each state $s \in S$ as:
\[
\text{SafeActions}(s) := \left\{ a \in A(s) \, \middle| \ 
\begin{aligned}
& x(s) < \infty ; \\
& \text{TotalCost}(s,a) \leq x(s); \\
& \text{TotalCost}(s,a) \leq \rcap
\end{aligned}
\right\}.
\]
\end{definition}


%The safe action map is defined as:
%\at{This is not a map. Also, it is never used, so it should be removed}
%\[
%\text{SafeActionsMap} := \setcond{s \in S}{\text{SafeActions}(s) \neq \emptyset}.
%\]

Based on this, we define the pruned product CMDPST $\mdpst[Z]_{\text{safe}}^{\times}$ as the sub-CMDPST of $\mdpst[Z]_{\text{pre}}$ where the action set at each state $s$ is restricted to $\text{SafeActions}(s)$.





\begin{lemma}
Let $\mdpst[Z]_{\text{safe}}^{\times}$ be the pruned product CMDPST constructed via the safe action set in Definition~\ref{safety definition}. 
Then, any path $\fpath^{\times}$ generated by a strategy over $\mdpst[Z]_{\text{safe}}^{\times}$ is guaranteed to be resource-safe, that is, it never exceeds the resource capacity $\rcap$ before reaching the winning region $W$.
\end{lemma}
\begin{proof}
We prove the result by showing that any strategy operating over $\mdpst[Z]_{\text{safe}}^{\times}$, by construction, cannot produce a path that violates the resource capacity constraint before reaching the target set $W$.

Let $\xi^{\times} = s_{0}^{\times} a_{0}^{\times} s_{1}^{\times} a_{1}^{\times} \cdots$ be an infinite path generated by a strategy $\sigma$ over $\mdpst[Z]_{\text{safe}}^{\times}$. Since the pruned model only allows actions from the set $\text{SafeActions}(s)$, it follows that each action $a_{t}^{\times}$ taken at state $s_{t}^{\times}$ satisfies the safety conditions defined in Definition~\ref{safety definition}.

In particular, for each transition $(s_{t}^{\times}, a_{t}^{\times})$, we have:
\[
\begin{aligned}
\text{TotalCost}(s_{t}^{\times}, a_{t}^{\times}) 
&:= C(s_{t}^{\times}, a_{t}^{\times}) + \max_{\Theta \in \mathcal{F}(s_{t}^{\times}, a_{t}^{\times})} \max_{s' \in \Theta} x(s') \\
&\leq x(s_{t}^{\times}) \leq \rcap.
\end{aligned}
\]
This implies that:
\begin{itemize}
    \item The immediate cost of each action is feasible;
    \item The pessimistic cost-to-go from all reachable successors remains within the safe bound;
    \item The accumulated cost along any worst-case path is strictly bounded by $\rcap$.
\end{itemize}

Moreover, since the pessimistic cost function $x(\cdot)$ is computed via value iteration assuming the worst-case nondeterministic transitions, any path respecting the safety constraints is conservative by design: it cannot lead to resource exhaustion before reaching the goal.

Therefore, under any strategy $\sigma$ over $\mdpst[Z]_{\text{safe}}^{\times}$, the accumulated cost along any path remains below $\rcap$ until the first visit to $W$. That is, all paths are resource-safe.
\end{proof}




\subsection{Strategy Synthesis}

After applying safety pruning to remove all actions that may cause resource exhaustion, we obtain a reduced model $\mdpst[Z]_{\text{safe}}^{\times}$ in which all paths are guaranteed to be resource-safe. As a result, the original hard constraint on energy consumption is now structurally encoded in the model.

We can therefore reformulate the original constrained optimisation problem as a probabilistic planning problem over the safe model. That is, we aim to compute an optimal stationary strategy $\sigma^*_{\text{pre}}$ such that:

\[
\sigma^*_{\text{pre}} \in \argmax_{\sigma^{\times} \in \Pi^{\times}} \prob_{\mdpst[Z]_{\text{safe}}^{\times}}^{\sigma^{\times}}(\Diamond W^{\times}).
\]



Then we synthesize a stationary strategy $\sigma^{\times}_{\text{pre}}$ that maximizes the probability of reaching the winning region $W^{\times}$ over the resource-safe product MDPST $\mdpst[Z]_{\text{safe}}^{\times}$.

Let $S_{\text{pre}} := S \setminus W^{\times}$ denote the set of non-accepting states. For each state $s \in S_{\text{pre}}$, we define the reachability value function $v(s)$ , initialized as:
\[
v(s) := 0; \qquad v(s) := 1,\quad \forall s \in W^{\times}.
\]

We perform value iteration over $\mdpst[Z]_{\text{safe}}^{\times}$. At each iteration and for each $s \in S_{\text{pre}}$, we update:
\begin{align*}
v(s) &\leftarrow \max_{a \in \text{SafeActions}(s)} \sum_{\Theta \in \mathcal{F}(s, a)} \mathcal{T}(s, a, \Theta) \cdot \min_{s' \in \Theta} v(s'), 
\end{align*}
where $a^*$ is the action maximizing the first expression. The operator $\min_{s' \in \Theta} v(s')$ accounts for the worst-case environment choice, and $\mathbb{E}$ denotes uniform expectation over $\Theta$.

The process iterates until the maximum change in both $v(s)$ falls below a given threshold. Once converged, we construct the strategy $\sigma^{\times}_{\text{pre}}$ by selecting for each state $s$ an action that maximizes the updated reachability value.

The output is a memoryless strategy $\sigma^{\times}_{\text{pre}}$ that is:
\begin{itemize}
    \item resource-safe (due to prior pruning),
    \item optimal with respect to reachability probability,
\end{itemize}



==> sections/minimize_consumption_with_a_certain_probability.tex <==
\section{Minimize Consumption with a Certain Probability}
In this section, we focus on minimizing the expected cost under a task satisfaction probability constraint. Specifically, the objective is to minimize the expected consumption from the initial state while ensuring that the $LTL_f$ specification is satisfied with at least a given probability threshold.

Following the approach in Section~4, we incorporate the $LTL_f$ formula into the original consumption MDPST by constructing a product MDPST $\mathcal{M}^\times$. Based on this construction, we identify the winning region $W$, which consists of:
\begin{itemize}
    \item target states that are reachable from the initial state even under the worst-case transition choices;
    \item and reload states that are reachable from the initial state and from which some target state is also reachable under worst-case transitions.
\end{itemize}

We now proceed to synthesize a strategy that ensures the system reaches the winning region $W$ with a probability no less than the given threshold $\delta$, while minimizing the expected accumulated cost during the execution.


Given an infinite path \(\xi^\times = s_0^\times a_0^\times s_1^\times a_1^\times \cdots\) of \(\mathcal{M}_{\text{sub}}^\times\) and the winning accepting region $W$, the total cost is defined as:

\[
\text{Cost}_{\text{pre}}(\xi^\times) = \sum_{t=0}^{T-1} C^\times (s_t^\times, a_t^\times)
\]

where \( T = \arg \min_t \{ s_t^\times \in W \} \) represents the first time that the path reaches $W$. Given a strategy \(\sigma^\times\) starting from \(s^\times\), the expected total cost induced by \(\sigma^\times\) is defined as:

\[
Q_{\text{pre}}(s^\times, W, \sigma^\times) := \mathbb{E}_{\xi^\times \in Q^{\sigma^\times}(s_0^\times)} \left[ \text{Cost}_{\text{pre}}(\xi^\times) \right]
\]
We define the problem as follows:

\textbf{Problem }  Given the product MDPST \(\mathcal{M}_{\text{sub}}^\times\), compute an optimal stationary prefix strategy \(\sigma_{\text{pre}}^*\) that solves the problem:

\[
\min_{\sigma^\times \in \Pi^\times} Q_{\text{pre}}(s_0^\times, W, \sigma^\times)
\]

subject to:

\[
\mathbb{P}_{\mathcal{M}_{\text{sub}}^\times}^{\sigma^\times} \left( \Diamond W \right) > \delta
\]

To solve this problem, we propose a three-step solution. First, we transform the finite-horizon constrained cost minimisation problem into an equivalent infinite-horizon one. Next, we reformulate the infinite-horizon constrained cost minimisation problem as an equivalent unconstrained sup-inf optimisation problem. Finally, we introduce an algorithm to approximate the optimal strategy prefix for the unconstrained sup-inf optimisation problem.

Given the product MDPST \(\mathcal{M}_{\text{sub}}^{\times}\) and the winning accepting region \(W\), we start by defining a modified MDPST \(\mathcal{Z}_{\text{pre}}\) of \(\mathcal{M}_{\text{sub}}^{\times}\) as

\[
\mathcal{Z}_{\text{pre}} = (S_{\text{pre}}, s_{0}^{\times}, A_{\text{pre}}, \mathcal{F}_{\text{pre}}, \mathcal{T}_{\text{pre}}, \mathcal{L}^{\times}, C_{\text{pre}},R_{\text{pre}},cap_{\text{pre}}),
\]

where \(S_{\text{pre}} = S^\times \setminus \{  s^{\times} \in \mathtt{Acc}^{\times} \wedge s^{\times} \notin W^{\times} \}\), \(A_{\text{pre}} = A^{\times} \cup \{\tau\}\) and \(\tau\) is a self-loop action. The set-valued nondeterministic transition function \(\mathcal{F}_{\text{pre}}\) is defined as i) \(\forall s \notin  W^{\times}\), \(\Theta \in \mathcal{F}_{\text{pre}}(s^{\times}, a^{\times})\) iff \(\Theta \in \mathcal{F}_{p}(s^{\times}, a^{\times})\) and \(\Theta \subseteq S_{\text{pre}}\) and ii) \(\forall s \in  W^{\times}\), \(\mathcal{F}_{\text{pre}}(s^{\times}, \tau) = s^{\times}\). The transition probability function is given by \(\mathcal{T}_{\text{pre}}(s^{\times}, a^{\times}, \Theta) = \mathcal{T}_{p}(s^{\times}, a^{\times}, \Theta)\). Finally, the cost function \(C_{\text{pre}}\) is defined by \(C_{\text{pre}}(s^{\times}, a^{\times}) = C^{\times}(s^{\times}, a^{\times}), \forall s \notin  W^{\times}\) and \(C_{\text{pre}}( W^{\times}, \tau) = 0, \forall s \in S_{\text{acc}}\).

The infinite-horizon total cost function \(\text{Cost}_{\text{pre}}\) for \(Z_{\text{pre}}\) is given by

\[\text{Cost}_{\text{pre}}(s_0^\times) = \sum_{t=0}^\infty C_{\text{pre}}(s_t^\times, a_t^\times).\] 

Then the expected total prefix cost induced by \(\sigma^\times\) of \(Z_{\text{pre}}\) is given by

\[\hat{Q}_{\text{pre}}(s_0^\times, \sigma^\times) := \text{Exp}_{\xi^\times \in \hat{\Omega}^{\sigma^\times}(s_0^\times)}[\text{Cost}_{\text{pre}}(\xi^\times)],\]

where \(\hat{\Omega}^{\sigma^{\times}}(s_{0}^{\times})\) is the set of all infinite paths of \(Z_{\text{pre}}\) generated by \(\sigma^{\times}\) from \(s_{0}^{\times}\).

It's straightforward to show that

\[\hat{Q}_{\text{pre}}(s_{0}^{\times},\sigma^{\times})=Q_{\text{pre}}(s_{0}^{\times},S_{\text{acc}}, \sigma^{\times})\]

since the cost of staying in \(S_{\text{acc}}\) is zero in \(Z_{\text{pre}}\).

Next we can reformulate Problem into an equivalent unconstrained sup-inf optimisation problem. The associated Lagrangian function is defined as

\begin{align*}
L(\sigma^{\times},\lambda) 
&= \lambda(\Pr_{\mathcal{M}_{\text{sub}}^{\times}}^{\sigma^{\times}}(\langle\rangle S_{\text{acc}})-\delta)-Q_{\text{pre}}(s_{0}^{\times},S_{\text{acc}},\sigma^{\times}) \\
&= \lambda(\Pr_{Z_{\text{pre}}}^{\sigma^{\times}}(\langle\rangle S_{\text{acc}})- \delta)-\hat{Q}_{\text{pre}}(s_{0}^{\times},\sigma^{\times}) \\
&= \lambda(\Pr_{Z_{\text{pre}}}^{\sigma^{\times}}(\langle\rangle W^{\times})- \delta)-\hat{Q}_{\text{pre}}(s_{0}^{\times},\sigma^{\times}),
\end{align*}


where \(\lambda\) is the Lagrangian multiplier.

Let

\[l^{*}:=\sup_{\sigma^{\times}\in\Pi^{\times}}\inf_{\lambda\geq 0}L(\sigma^{\times},\lambda).\]

Following the argument in ~\cite{boyd:04}, one can show that Problem is equivalent to the sup-inf optimisation problem . That is, if an optimal solution \(\sigma^{*}_{\text{pre}}\) exists in Problem, then \(\sigma^{*}_{\text{pre}}\) is a maximiser. The optimal value of Problem is equal to \(l^{*}\).Then we propose to use the Exponential Gradient Algorithm (Algorithm ~\ref{Exponential Gradient Algorithm}) to approximately solve the optimal strategy for the sup-inf optimization problem.


\begin{algorithm}
\caption{Exponential Gradient Algorithm}
\label{Exponential Gradient Algorithm}
\begin{algorithmic}[1]
\State \textbf{Initialize:} \(\lambda_{1} = M/2\)
\For{\(k = 1, \ldots, K\)}
    \State \(\sigma_{k} \leftarrow \text{OPT}(\mathcal{Z}_{\text{pre}}, \lambda_{k})\)
    \State \(p_{k} \leftarrow \text{EVAL}(\mathcal{Z}_{\text{pre}}, \sigma_{k})\)
    \State \(\lambda_{k+1} \leftarrow M \dfrac{\lambda_{k} e^{-\eta (p_{k} - \lambda)}}{M + \lambda_{k} (e^{-\eta (p_{k} - \lambda)} - 1)}\)
\EndFor
\State \(\bar{\sigma}_{\text{pre}} = \dfrac{\sum_{i=1}^{K} \sigma_{k}}{K}\), \(\bar{\lambda} = \dfrac{\sum_{i=1}^{K} \lambda_{k}}{K}\)
\end{algorithmic}
\end{algorithm}



Algorithm~\ref{Exponential Gradient Algorithm} takes the prefix MDPST \(\mathcal{Z}_{pre}\), the upper bound \(M\) of the Lagrangian multiplier, the number of iterations \(K\), and a scaling parameter \(\eta\) for the exponential function as input. The output is the approximation solution \(\bar{\sigma}_{pre}\) to problem. We begin by initialising the Lagrangian multiplier \(\lambda = M/2\). At each iteration \(k\) , one first solves an unconstrained optimisation problem OPT\((Z_{pre}, \lambda_k)\). After that, one can compute the probability of robust satisfying the LTL formula \(\varphi\) given the optimal strategy \(\sigma_k\) obtained at the previous step (i.e., \(p_k\)), using the evaluation function EVAL\((Z_{pre}, \sigma_k)\) . Finally, we update the Lagrangian multiplier \(\lambda_{k+1}\) using an exponential function .

The unconstrained optimisation problem OPT\((Z_{pre}, \lambda_k)\) and the evaluation function EVAL\((Z_{pre}, \sigma_k)\) are further detailed in the following.

Let us define a task satisfaction value function \(\hat{V}_{pre}^{sat}\) for \(Z_{pre}\) as
\begin{align*}
\hat{V}_{pre}^{sat}(s^{\times}) 
&= \max_{\sigma^{\times}(s^{\times})} \min_{\gamma^{\times}} \Bigl\{ \\
&\quad \Pr_{Z_{pre}}\bigl( \bigl\{ \xi^{\times} \in \Omega_{\sigma^{\times}(s^{\times}), \gamma^{\times}}^{Z_{pre}}(s^{\times}) \bigm| \\
&\quad \mathcal{L}^{\times}(\xi^{\times}) \models \hat{\nabla}W^{\times} \bigr\} \bigr) \Bigr\},
\end{align*}
which represents the robust maximal probability of reaching \(W^{\times}\) from \(s^{\times}\). In addition, we define a prefix cost value function for \(Z_{pre}\) as
\[
\hat{V}_{pre}^{cost}(s^{\times}) = \min_{\sigma^{\times}} \{\hat{Q}_{pre}(s^{\times}, \sigma^{\times})\}.
\]

Notice that for states \(s^{\times} \in S_{acc}\), one has that \(\hat{V}_{pre}^{cost}(s^{\times}) = 0\) and for states \(s^{\times} \in W^{\times}\), one has that \(\hat{V}_{pre}^{sat}(s^{\times}) = 1\). In addition, for states \(s^{\times} \in S_{pre} \setminus S_{acc}\), one has that
\begin{align*}
\hat{V}_{pre}^{cost}(s^{\times}) 
&= \min_{a^{\times} \in A_{pre}(s^{\times})} \biggl\{ C_{pre}(s^{\times}, a^{\times}) \\
&\quad + \sum_{\Theta \in \mathcal{F}_{pre}(s^{\times}, a^{\times})} T_{pre}(s^{\times}, a^{\times}, \Theta) \\
&\quad \cdot \frac{\sum_{s^{\prime} \in \Theta} \hat{V}_{pre}^{cost}(s^{\prime})}{|\Theta|} \biggr\}.
\end{align*}
For states \(s^{\times} \in S_{pre} \setminus W^{\times}\), one has that
\begin{align*}
\hat{V}_{pre}^{sat}(s^{\times}) 
&= \max_{a^{\times} \in A_{pre}(s^{\times})} \biggl\{ \\
&\quad \sum_{\Theta \in \mathcal{F}_{pre}(s^{\times}, a^{\times})} T_{pre}(s^{\times}, a^{\times}, \Theta) \\
&\quad \cdot \min_{s^{\prime} \in \Theta} \{\hat{V}_{pre}^{sat}(s^{\prime})\} \biggr\}.
\end{align*}

With the task satisfaction and prefix cost value functions \(\hat{V}_{pre}^{sat}\) and \(\hat{V}_{pre}^{cost}\), one can now define the unconstrained optimisation problem OPT\((Z_{pre}, \lambda_k)\), which is given by
\begin{align*}
\sigma_k &= \text{OPT}(Z_{pre}, \lambda_k) \\
&= \arg \inf_{\sigma^{\times}} \left\{ \hat{V}_{pre}^{cost}(s_{0}^{\times}) - \lambda_k (\hat{V}_{pre}^{sat}(s_{0}^{\times}) - \delta) \right\}.
\end{align*}

The evaluation function EVAL\((\mathcal{Z}_{pre},\lambda_{k})\) is then given by
\[
\text{EVAL}(\mathcal{Z}_{pre},\lambda_{k}) = \Pr_{\mathcal{Z}_{pre}}^{\sigma_{k}}(\diamondsuit W^{\times}),
\]

Note that both \(\text{OPT}(\mathcal{Z}_{pre},\lambda_{k})\) and EVAL\((\mathcal{Z}_{pre},\lambda_{k})\) can be obtained using (robust) value iteration methods.

The following theorem shows that the strategy \(\bar{\sigma}_{pre}\) obtained from Algorithm~\ref{Exponential Gradient Algorithm} is an \(\epsilon\)-optimal strategy for Problem.

\begin{theorem}
If \(\eta = \sqrt{\dfrac{\log 2}{2K^{2}M^{2}}}\), the strategy \(\bar{\sigma}_{pre}\) returned by Algorithm~\ref{Exponential Gradient Algorithm} satisfies
\begin{align*}
&\Pr_{\mathcal{M}^{\times}_{sub}}^{\bar{\sigma}_{pre}}(\diamondsuit S_{acc}) \geq \delta + \frac{C^{*} - 2M\sqrt{2\log 2/K}}{M}, \\
&Q_{pre}(s_{0}^{\times}, S_{acc}, \bar{\sigma}_{pre}) \leq C^{*} + 2M \sqrt{2\log 2/K},
\end{align*}
where \(C^{*}\) is the minimal achievable cost in Problem.
\end{theorem}
